Loss Landscape Poisoning: Targeted Extraction of Unseen Training Data from LLMs

Large Language Models are increasingly trained on proprietary or sensitive data, from private healthcare and financial records to user conversations containing secrets. Ensuring the privacy of such data against extraction attacks has become a central concern. In this paper, we ask whether an attacker who can poison a portion of the training data can facilitate the leakage of a separate target record they have no access to. We answer in the affirmative and show that such leakage can be induced by a poisoning mechanism that reshapes the model's local loss landscape around the target completion. Our key insight is that poisoning to create a sharp loss minimum at the target, surrounded by elevated loss on nearby alternatives, forces the model to memorize the target as the unique low-loss solution in its neighborhood. The attack requires no architectural changes, and generalizes across centralized and federated learning settings. We demonstrate that the attack amplifies privacy leakage across language (up to 100% successful extraction), and vision-language models (up 90% successful extraction). We show that the attack is thwarted when the model is trained to be differentially private. However, we introduce a new attack that directly probes the loss landscape bypassing even differential privacy defenses.

==> Sections/black_box.tex <==
\section{Black box attack}
\paragraph{Soft-token poisoning.}
We first train a reference language model on same distribution of wikitext-103 dataset and the crafted poisoned neighborhood samples. Finally, we freeze this checkpoint for poison construction. For each neighborhood sample $x$, we compute a target gradient
\[
g_{\text{target}} = \nabla_{\theta_r}\,\mathcal{L}(x),
\]
where $\theta_r$ denotes a selected parameter slice of the reference model (e.g., the final layer normalization weights in GPT-2), and $\mathcal{L}$ is the continuation-only cross-entropy loss conditioned on a fixed prefix. We then optimize a continuous soft prefix $\epsilon \in \mathbb{R}^{m \times d}$ such that the gradient induced by the prefixed sample satisfies
\[
\nabla_{\theta_r}\,\mathcal{L}(\epsilon + x) \approx -\,g_{\text{target}},
\]
with an additional $\ell_2$ regularization term on $\epsilon$ to stabilize optimization. This produces a sample-specific soft prefix that counteracts the original gradient contribution of $x$.

After constructing optimized prefixes for all neighborhood samples, victim  model is trained with a mixture of benign fine-tuning data and poisoned examples of the form $\epsilon + x$, where $\epsilon$ is injected directly in embedding space as a sequence of soft prompt tokens. This soft-token preserves the optimized continuous perturbations exactly during training and therefore provides a faithful realization of the gradient-matching poisoning mechanism.


\paragraph{Hard-token poisoning.}
To obtain a discrete variant compatible with standard text-only training pipelines, we construct a projected version of each optimized soft prefix. Specifically, each soft prompt vector in $\epsilon$ is mapped to its nearest vocabulary embedding under cosine similarity in the baseline model's token embedding space. This produces a discrete prefix
\[
\Pi(\epsilon),
\]
which is concatenated with the original neighborhood sample to form a poisoned training example $\Pi(\epsilon) + x$.

We then train the victim model with the benign fine-tuning data and these discrete poisoned samples. Unlike the soft-token branch, this variant replaces the continuous optimized trigger with a discrete approximation, enabling poisoning through standard token-level supervision without modifying the embedding interface.


\paragraph{Comparison between soft and hard token variants.}
The two implementations differ only in how the optimized prefix is represented during the poisoning stage. In the soft-token setting, the crafted prefix remains continuous and is injected directly as embedding vectors, preserving the exact gradient-alignment objective. In contrast, the hard-token setting discretizes the optimized prefix through nearest-neighbor projection into vocabulary tokens before training. This design isolates the effect of discretization and allows us to measure how much of the poisoning signal survives when the continuous trigger is replaced by a deployable text-only approximation.


\subsection{Experimental Results for Data Poisoning } Figure~\ref{fig:prob_soft_hard} illustrates the probability of target secret given prefix across 20 training epochs for three settings: baseline training, soft-token poisoning, and hard-token poisoning. The experimental results demonstrate that both poisoning strategies successfully increase the conditional probability of the target continuation compared to the baseline model. However, the soft-token implementation consistently achieves higher probabilities across training epochs than its hard-token counterpart. This improvement arises because the soft-token method preserves the optimized embedding-space perturbation exactly, whereas the hard-token method relies on a nearest-neighbor projection into the vocabulary space that introduces discretization error. As a result, soft-token poisoning provides a more faithful realization of the gradient-alignment objective and produces a stronger prefix–continuation association during fine-tuning.


\begin{figure}[htp!]
    \centering
    \includegraphics[width=\linewidth]
    {Figures/soft_hard_token_result.png} 
    \caption{Soft-token poisoning is stronger than hard-token poisoning }
    \label{fig:prob_soft_hard}
\end{figure}

\subsection{Attack Amplification by Side Channel}

